Spatial Signal Design for Positioning via End-to-End Learning

This letter considers the problem of end-to-end learning for joint optimization of transmitter precoding and receiver processing for mmWave downlink positioning. Considering a multiple-input single-output (MISO) scenario, we propose a novel autoencoder (AE) architecture to estimate user-equipment(UE) position with multiple base-stations (BSs) and demonstrate that end-to-end learning can match model-based design, both for angle of departure (AoD) and position estimation, under ideal conditions without model deficits and outperform it in the presence of hardware impairments.

==> Other/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> new pics/BS_scheme_one_column.tex <==
  \begin{tikzpicture}
    \node(image) [anchor=south west] at (2,0)  {\includegraphics[width=0.46\linewidth
    ,height=5cm]{new pics/bs.pdf}
    };
    %\draw [help lines] (0,0) grid (6,4);;
    \node at (4.6,4.9){UE};
    \node at (5.7,4.85){$\bm{p}$};
    \node at (6.4,2.8){${\theta_2}$};
    \node at (6.3,2.3){${\psi_2}$};
    \node at (6,0.5){BS $2$};
    \node at (7.7,0.6){$\ldots$};
    \node at (10.8,1){$x$};
    \node at (4,0.5){BS $1$};
    \node at (4,2.5){${\theta_1}$};
    \node at (3.1,2.8){${\psi_1}$};
    \node at (10,0.5){BS $I$};
    \node at (8.8,2.3){${\theta_I}$};
    \node at (9.5,2.5){${\psi_I}$};
    \end{tikzpicture}









%   \begin{tikzpicture}
%     \node(image) [anchor=south west] at (0,0)  {\includegraphics[width=1\linewidth]{tikz examplesfiles/bs.pdf}
%     };
%     %\draw [help lines] (0,0) grid (6,4);;
%     \node at (4.8,4.6){UE};
%     \node at (6.7,2.4){${\theta_2}$};
%     \node at (7.3,2.6){${\psi_2}$};
%     \node at (8.1,0.8){BS$2$};
%     \node at (9,1.2){$\boldsymbol{x}$};
%     \node at (1.1,0.8){BS$1$};
%     \node at (2.4,2.65){${\theta_1}$};
%     \end{tikzpicture}

==> new pics/RMSE_AOD_MC.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}[every node/.append style={font=\small}]

\begin{axis}[%
width=0.8\linewidth,
height=3cm,
at={(0.758in,0.485in)},
scale only axis,
xmin=-5,
xmax=30,
xlabel style={font=\color{white!15!black}},
xlabel={SNR [dB]},
ymode=log,
ymin=0.01,
ymax=10,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={RMSE [$^{\circ}$]},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
ylabel style={yshift=-0.3cm},
xlabel style={yshift=0.3cm},
legend columns=2,
legend style={legend cell align=left, align=left, draw=white!15!black,font=\small,nodes={scale=0.8, transform shape}},
tick label style={font=\tiny}
]
\addplot [color=mycolor1, dashed, line width=2.0pt, mark size=3.0pt, mark=o, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
-5	3.58044707111289\\
0	2.3875758735593\\
5	1.43753393234724\\
10	0.627552334270315\\
15	0.457326403427969\\
20	0.268261345116908\\
25	0.214940831116165\\
30	0.210711434233994\\
};
\addlegendentry{benchmark RMSE}

\addplot [color=mycolor2, dashed, line width=2.0pt, mark size=3.0pt, mark=o, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
-5	2.07934464048582\\
0	0.94700930059104\\
5	0.278352378212025\\
10	0.137761760387381\\
15	0.0768490629695729\\
20	0.0450537746935926\\
25	0.0246459944488468\\
30	0.0136744688465832\\
};
\addlegendentry{learned RMSE}

\addplot [color=mycolor3, line width=2.0pt]
  table[row sep=crcr]{%
-5	1.10552596123914\\
0	0.621682934075553\\
5	0.349598004996271\\
10	0.196593405413505\\
15	0.110552596123914\\
20	0.0621682934075553\\
25	0.0349598004996271\\
30	0.0196593405413505\\
};
\addlegendentry{benchmark CRB}

\addplot [color=mycolor4, line width=2.0pt]
  table[row sep=crcr]{%
-5	0.795978692092182\\
0	0.447611712534398\\
5	0.251710563597315\\
10	0.141547251897724\\
15	0.0795978692092182\\
20	0.0447611712534398\\
25	0.0251710563597315\\
30	0.0141547251897724\\
};
\addlegendentry{learned CRB}

\end{axis}
\end{tikzpicture}%
